Online Improper Learning with an Approximation Oracle

We revisit the question of reducing online learning to approximate optimization of the offline problem. In this setting, we give two algorithms with near-optimal performance in the full information setting: they guarantee optimal regret and require only poly-logarithmically many calls to the approximation oracle per iteration. Furthermore, these algorithms apply to the more general improper learning problems. In the bandit setting, our algorithm also significantly improves the best previously known oracle complexity while maintaining the same regret.

==> OMD.tex <==
\section{Efficient Online Mirror Descent on $\reals^d_+$}\label{sec:OMD}

In this section, we will exhibit a more efficient online gradient descent algorithm when the domain of the linear loss functions are contained in its self dual cone. This algorithm also achieves the optimal regret, $O(\sqrt{T})$, like the previous OGD based algorithms. Note this is slightly better the regret bound CMWU, $O(\sqrt{Td})$. However the previous algorithm is more general because it doesn't have the restriction on loss function's domain.  Still, there are lots of interesting domains $W$ falling into this restriction, such as the non-negative orthant, $\reals^d_+$, semi-definite positive matrix cone, and Lorentz cone $L_{d+1}=\{(x,t)\in \reals^{d+1}:\|x\|_2\leq t\}$. For simplicity, we state our results with the non-negative orthant, and give a faster algorithm for the problem of $\alpha$ -regret minimization in online linear optimization [cite][cite]. Moreover, our approach can be generalized to to implement Online Mirror Descent with $\alpha$ -approximation oracles.% which gives us an efficient semi-bandit algorithm with optimal $\sqrt{dT}$ regret, while the regret of OGD in [cite][cite] is suboptimal, $O(d\sqrt{T})$, and those algorithms uses more oracle calls per iteration.  






\subsection{The algorithm sketch} 

\begin{definition}[Infeasible projection oracle]
An \emph{infeasible projection operator} over $\ch(\alpha \K)$ is defined as a procedure that given input $y \in \reals_+^d$ and tolerance $\epsilon>0$ produces a tuple $\widetilde{\Pi}_\K(y,\epsilon) = (y',\bp=\{p_i\}_{i=1}^k,\bv=\{v_i\}_{i=1}^k) $ that satisfies:
\begin{enumerate}
\item It's closer to $\alpha \K$ as compared to $y$
$$ \forall y^* \in \alpha \K , \  B_\R(y^*,y') \leq B_\R(y^*,y)   $$ 

\item $v_i\in \K,\ \forall i=[k]$. And $\{p_i\}_{i=1}^k$ represents a convex combination of  $\bv$ which `almost' dominates $x'$. In other words, there exists $c\in \reals^d_+$, s.t.
$$  \| \sum_{i=1}^k p_i v_i + c - y'  \| \leq \eps $$

\end{enumerate}
\end{definition}

We later show that this projection $y' = \widetilde{\Pi}_\K(x,\epsilon) $ can be computed using $O(d \ln \frac{1}{\eps})$ calls for $\alpha$ approximated minimization oracle $\O_{\K,\alpha\K}$. 
Given the approximate infeasible projection operator, we can apply OMD as follows:
\begin{algorithm}
\caption{Online mirror descent with approximate infeasible projection.}
\label{alg:OMD}
\begin{algorithmic}[1]
	\STATE \textbf{Input:} Learning rate $\eta>0$, tolerance $\epsilon$.
	\STATE $y_1=0$.
	\FOR{$t=1$ to $T$}
    	\STATE Let $(x_{t},\bv_{t},\bp_{t})$ be the output of $\widetilde{\Pi}_\K (y_{t},\epsilon) $,
		\STATE play $v^t_i$ according to distribution $\bp^t$, observe $f_t$.
		\STATE update $\nabla \R(y_{t+1}) \leftarrow \nabla \R (x_t) - \eta f_t $ 
	\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:OMD_regret}
For any learning rate $\eta>0$, tolerance $\epsilon>0$ and any loss sequence $\{f_t\}_{t=1}^T\in (\reals^d_+\cap B(0,L))^T$, and domain $\K\in \reals^d_+\cap B(0,R)$, assuming the regularizer $\R$ is seperable,  Algorithm $\ref{alg:OMD}$ has the following regret guarantee: $\forall x^*\in \K$,
\[
\alpha-Reg_T = \sum_{t=1}^T f_t^\top (x_t)-\alpha f_t(x^*)\leq \frac{1}{\eta}\left(B_\R(y^*,x_1)+\sum_{t=1}^T B_\R^*(\nabla \R(x_t)-\eta f_t,\nabla \R(x_t))\right)+ TL\epsilon.
\]

using at most $3d\ln \frac{R}{\epsilon}$ calls of oracle $\O_{\K,\K^*}$.

In particular, setting $\epsilon = \frac{1}{TL}$, $\eta = $, picking $R$ 1- strongly convex, we have

\[
\alpha-Reg_T = \sum_{t=1}^T f_t^\top (x_t)-\alpha f_t(x^*)\leq \frac{B_\R(y^*,x_1)}{\eta} + T\eta L^2+ 1=L\sqrt{T B_\R(y^*,x_1)}+1,
\]

using at most $3d\ln (TLR)$ calls of oracle $\O_{\K,\K^*}$.
\end{theorem}


\begin{proof} 
First, let's relate the regret of $x_t$ to that of playing distribution over $v^t_i$, but that is given by the third property of the approximate projection and Lipschitz property of $f_t$, namely
$$ f_t( \E_i v^t_i) - f_t(x_t - c) \leq f_t(\E_i v^t_i + c - x_t ) \leq L\epsilon $$ 
Thus by non-negativity of $f_t$, 
\begin{equation} \label{eqn:shalom}
f_t( \E_i v^t_i) \leq  f(x_t)+L\epsilon
\end{equation}



Let $x^* \in \K$ be any point, and $y^* = \alpha x^* \in \alpha \K$.  We make use of the following property of Bregman divergences:
$$ (x-y)^\top (\nabla \R(z) - \nabla \R(y) ) = B_\R( x,y) - B_\R( x,z) + B_\R(y,z)  $$ 
Thus,

\begin{eqnarray*}
\sum_t f_t(x_t) - f_t(y^*) & \leq \sum_t f_t (x_t - y^* ) \\
& = \sum_t  \frac{1}{\eta} \left( \nabla \R( y_{t+1} )  - \nabla \R( x_t) \right) (x_t - y^*) & \mbox{alg definition}  \\
& = \sum_t \frac{1}{\eta} \left[ B_\R ( y^* , x_t) - B_\R(y^* , y_{t+1} ) + B_\R(x_t , y_{t+1} ) \right]  \\
& \le \sum_t  \frac{1}{\eta} \left[ B_\R ( y^* , x_t) - B_\R(y^* , x_{t+1} ) + B_\R(x_t , y_{t+1} ) \right]  & \mbox{property (1) of projection} \\
& \leq   \frac{1}{ \eta} [B_\R ( y^* , x_1) + B_{\R^*}(\nabla \R(y_{t+1}),\nabla \R(x_t))]  & \mbox{ Property of Bregman's divergence } \\
& \leq \frac{1}{ \eta} [B_\R ( y^* , x_1) + B_{\R^*}(\nabla \R(x_t)-\eta f_t,\nabla \R(x_t)) ]
\end{eqnarray*}


and thus the expected $\alpha$ regret of the algorithm can be bounded by,
\begin{eqnarray*}
\mbox{$\alpha$-Regret} & = \sum_t \E [f_t v^t_i] -  \sum_t f_t y^* \\
 & \leq \sum_t f_t(x_t) -  \sum_t f_t(y^*) + TL\epsilon  & \mbox{ equation \eqref{eqn:shalom}} \\
& \leq  \frac{1}{ \eta} [B_\R(y^*,x_1) +  B_{\R^*}(\nabla \R(x_t)-\eta f_t,\nabla \R(x_t))] + TL\epsilon
\end{eqnarray*}

Note that for $\frac{1}{\beta}$ -strongly convex functions, its bregman divergence is $\beta$ -smooth. By our 1-strongly convex assumption for $\R$, it holds that 
\[ B_{\R^*}(\nabla \R(x_t)-\eta f_t,\nabla \R(x_t))\leq \eta^2\|f_t\|^2\leq \eta^2 L^2.\] This concludes the proof.
\end{proof}

\subsection{Construction of the infeasible projection oracle}



In this section we prove Theorem \ref{thm:projection} concerninng approximate projections, computed by the algorithm below. 

\begin{theorem} \label{thm:projection}
Algorithm \ref{alg:infeasible_projection} below computes the projection $y' = \widetilde{\Pi}_\K(y) $ using $O(d \log \frac{1}{\eps})$ oracle calls. The point $u$ satisfies: 
\begin{enumerate}
\item
$ \forall y^* \in \alpha\K \ , \  B_\R(x,y') \leq B_\R(x,y)   $
\item $v_i\in \K,\ \forall i=[k]$. And $\{p_i\}_{i=1}^k$ represents a convex combination of  $\bv$ which `almost' dominates $x'$. In other words, there exists $c\in \reals^d_+$, s.t.
$$  \| \sum_{i=1}^k p_i v_i + c - y'  \| \leq \eps $$
\end{enumerate}
\end{theorem}



\begin{algorithm}
\caption{(Infeasible) Projection onto CH($\alpha K$), $\widetilde{\Pi}_\K(y,\epsilon) $    }\label{alg:infeasible_projection}
\begin{algorithmic}[1]
	\STATE \textbf{Input:} Point $y\in \reals^d$, tolerance $\epsilon>0$, $\alpha$-approximation oracle $\O_{\K,\alpha\K}$. 
	\STATE \textbf{Output:} $y' = y_{k+1}$,$(v_1,\ldots,v_k)$, $(p_1,\ldots,p_k)$, where $\bp$ is a distribution on $\bv$ and $k=3d\ln \frac{(\alpha +1)R}{\epsilon}$.
    \STATE $W_1 = \mathbb{R}^d_+\cap B(0,1)$, $y_1 = y$.
	\FOR{$t=1\ldots k$}
		\STATE $w_t = \int_{w\in W_t}w \dw$. 
		\STATE $v_t = \O_{\K,\K^*}(w_t)$.
		%\STATE $x_{t+1} = x_{t} + \max\{0,w_t^T(p_t-x_t)\}\frac{w_t}{\|w_t\|^2}$. \mbox{Now we have $w_{t}^T(p_t-x_{t+1})\leq 0$}
        \STATE $y_{t+1} = \argmin\limits_{y:w_t^T(y-v_t)\geq0} B_\R(y,y_t)$ \zhiyuan{Could be solved by Convex optimization}
		\STATE $W_{t+1} = W_t \cap \{w| w^T(p_t-y_{t+1}) > 0\}$. \quad  \zhiyuan{ gravity center is on the cutting plane}
	\ENDFOR
    \STATE Solve $\D(y_{k+1},\bv,\reals^d_+)$ for $\bp$.
\end{algorithmic}
\end{algorithm}

Now we will prove \cref{thm:projection}. The first properties holds because of generalized Pythagorean theorem, namely $\forall y^*\in \alpha \K$, $ B_\R(y^*,y_{t+1})\leq B_\R(y^*,y_t)$. For the second property, we have the following lemmas:

\begin{lemma}
If $\R(\x)=\sum_{i=1}^d r_i(x^i)$, where $r_i$ are convex functions. Then $\forall 1\leq t\leq k$, $y_{t+1}-y_t\in \reals^d_+$.
\end{lemma}

\begin{proof}
By definition, $y_{t+1} = \argmin\limits_{y:w_t^T(y-v_t)\geq0} B_\R(y,y_t)$. By optimality condition, $\nabla B_\R(y,y_t)|_{y=y_{t+1}} = \nabla \R(y_{t+1})-\nabla \R(y_t) = C w$, for some $C>0$. Since $\R(x)$ is separable, we have $0\leq Cw_i= r_i'(y_{t+1}^i)- r_i'(y_t^i)$. Note that $r_i'$ nondecreasing, thus $y_{t+1}^i-y_t^1\geq 0$, $y_{t+1}-y_t\in \reals^d_+$.
\end{proof}
\begin{lemma}
\[\forall w\in W_1\setminus W_{k+1},\ \exists v_i, \textrm{ s.t. } w^T(v_i-y_{k+1})\leq 0.\]
\end{lemma}

\begin{proof}
$\forall w\in W_1\setminus W_{k+1}$, $\exists t$, s.t. $w^T(v_t-y_{t+1})\leq 0$. Notice that $\forall s$, $y_{s+1}-y_{s}\in \mathbb{R}^d_+$ and $W_1\subseteq \mathbb{R}^d_+$, we have $w^T(v_t-y_{k+1}) \leq w^T(v_t-y_{t+1})\leq 0$.
\end{proof}

Using a similar argument in \lemmaref{lem:cutting_plane}, we have the following lemma.

\begin{lemma}
    \[\forall w\in \mathbb{R}^d_+, \|w\|=1,\ \exists v_i, \textrm{ s.t. } w^T(v_i-y_{k+1})\leq \epsilon.\]
\end{lemma}


By \lemmaref{lem:equivalence}, we have $\exists c \in \reals^d_+, \bp\in \Delta^{d-1}$,
$ \|\sum_{i=1}^k p_iv_i+c-y_{k+1}\|\leq \epsilon$. This concludes the proof the second property in \cref{thm:projection}.


\subsection{$\alpha$-approximation algorithms for semi-bandit setting}

\begin{theorem}
Assuming $\K\subset \{0,1\}^d$, and if $x\in \K$ then $\forall y\succeq x$, $y\in \K$. For any learning rate $\eta>0$, tolerance $\epsilon>0$ and any loss sequence $\{f_t\}_{t=1}^T\in (([0,1])^d)^T$, setting $\R(x)=\sum_{i=1}^dx_i(\ln x_i-1)$, Algorithm \ref{alg:semi_bandit} has the following regret guarantee: $\forall x^*\in \K$,

\[\E[\alpha-R_T]=\E[\sum_{t=1}^Tf_t^\top(x_t-\alpha^* x^*)]=\frac{d(1+\alpha\ln\alpha)}{\eta}+ \eta d\alpha\]
\end{theorem}
\begin{algorithm}
\caption{Online stochastic mirror descent with negative entropy for semi-bandit}
\label{alg:semi_bandit}
\begin{algorithmic}[1]
	\STATE \textbf{Input:} Learning rate $\eta>0$, tolerance $\epsilon$, $\alpha$- approximation oracle $\O_{\K,\alpha\K}$.
	\STATE $y_1=0$.
	\FOR{$t=1$ to $T$}
    	\STATE Let $(x_{t},\bv_{t},\bp_{t})$ be the output of $\widetilde{\Pi}_\K (y_{t},\epsilon) $,
		\STATE play $v^t_i$ according to distribution $\bp^t$, observe $f_t$.
		\STATE update $\nabla \R(y_{t+1}) \leftarrow \nabla \R (x_t) - \eta f_t $ 
	\ENDFOR
\end{algorithmic}
\end{algorithm}
\zhiyuan{To be continued}
% We also have the following lemma.

% \begin{lemma}\label{lem:equivalence}
% Fix $x\in \mathbb{R}^d_+$, and a set of vectors $\tv=(v_1,\ldots,v_k)$,$p_i\in\mathbb{R}^d_+$, the following two things are equivalent:
% \begin{itemize}
%     \item[(A)] $\exists a_i\leq 0, \sum_{i=1}^{k}p_i=1$ and $c\in \mathbb{R}^d_+$, s.t. $\|\sum_ip_iv_i+c-x\|\leq \epsilon$.
%     \item[(B)] $\forall w\in \mathbb{R}^d_+, \|w\|=1$, $\exists v_i$, s.t.  $w^T(v_i-y)\leq \epsilon$.
% \end{itemize}
% \end{lemma}

% \begin{proof}
% \ 

% \begin{itemize}
%     \item $(A)\to (B)$: \[\forall w\in \mathbb{R}^d_+,\ \min_i w^T(v_i-x)\leq w^T(\sum_i p_iv_i-x)\leq w^T(\sum_i p_iv_i+c-x)\leq |\sum_i p_iv_i+c-x|\leq \epsilon.\]
%     \item $(B)\to (A)$: Let $\ba^*,c^*= \argmin_{\ba,c}\|\sum_{i}p_iv_i+c-x\|$.
%     If the ith component of $\sum_{i}p_iv_i+c-x$ is negative, let $c'=c+\epsilon \be_i$, we have 
%     \[\|\sum_ip^*_iv_i+c'-x\|\leq \|\sum_ip^*_iv_i+c^*-x\|,\]
%     for $\epsilon$ small enough. 
    
%     Thus $\sum_{i}p^*_iv_i+c^*-x\in \mathbb{R}^d_+$. Let $w = \frac{\sum_{i}p^*_iv_i+c^*-x}{\|\sum_{i}p^*_iv_i+c^*-x\|}$. By optimality condition,  $w^T(\sum_{i}p^*_iv_i+c^*-x)\leq \min_i w^T(v_i-x)\leq \epsilon$.
% \end{itemize}

% \end{proof}


